Accelerating TinyML Inference on Microcontrollers through Approximate Kernels

The rapid growth of microcontroller-based IoT devices has opened up numerous applications, from smart manufacturing to personalized healthcare. Despite the widespread adoption of energy-efficient microcontroller units (MCUs) in the Tiny Machine Learning (TinyML) domain, they still face significant limitations in terms of performance and memory (RAM, Flash). In this work, we combine approximate computing and software kernel design to accelerate the inference of approximate CNN models on MCUs. Our kernel-based approximation framework firstly unpacks the operands of each convolution layer and then conducts an offline calculation to determine the significance of each operand. Subsequently, through a design space exploration, it employs a computation skipping approximation strategy based on the calculated significance. Our evaluation on an STM32-Nucleo board and 2 popular CNNs trained on the CIFAR-10 dataset shows that, compared to state-of-the-art exact inference, our Pareto optimal solutions can feature on average 21% latency reduction with no degradation in Top-1 classification accuracy, while for lower accuracy requirements, the corresponding reduction becomes even more pronounced.

==> Tables/related.tex <==
\begin{table}[t!]
\setlength\tabcolsep{5.3pt}
\renewcommand{\arraystretch}{1.3}
\scriptsize
\caption{Qualitative comparison of related frameworks.}
\begin{threeparttable}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\textbf{Framework} &
  \multicolumn{1}{l|}{\textbf{Orthog.\tnote{1}}} &
  \multicolumn{1}{l|}{\textbf{Customized\tnote{2}}} &
  \multicolumn{1}{l|}{\textbf{AC}} &
  \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}c@{}}Resource \\ Utilization\tnote{3}\end{tabular}}} &
  \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}c@{}}Acc - Latency\\ Trade-off\end{tabular}}} \\ \hline \hline
CMSIS-NN      & \cmark & \xmark  & \xmark  & \xmark  & \xmark     \\ \hline
X-CUBE-AI     & \xmark  & \cmark & \xmark  & $\approx$  & $\approx$ \\ \hline
TinyEngine    & \cmark & \cmark & \xmark  & \xmark  & \cmark     \\ \hline
CMix-NN       & \cmark & \xmark  & \cmark & \cmark  & \cmark    \\ \hline
MicroTVM      & \xmark  & \cmark & \xmark  & \xmark  & \xmark     \\ \hline \hline
\textbf{Ours} & \cmark & \cmark & \cmark & \cmark & \cmark    \\ \hline
\end{tabular}
\begin{tablenotes}\scriptsize
\item[] $^1$Orthogonal with other frameworks/techniques.
$^2$Customized code for specific models.
$^3$Efficient utilization of resources
\vspace{-2ex}
\end{tablenotes}
\end{threeparttable}
\label{tab:related}
\end{table}

==> background.tex <==
\section{Background \& Related Work}
% \blue{
% \textbf{Length: 0.5 pages. Figures: 0}
% \begin{itemize}
%     \item Related Works: pruning works, quantization (see mcunetv2), explain our orthogonal technique to existing libraries and frameworks.
% \end{itemize}
% }

\input{Tables/related}

Research in the deployment of deep inference networks in microcontrollers is increasingly growing with numerous frameworks targeting the widely used ARM Cortex-M MCUs and trying to bridge the gap posed by computational and memory limitations. 

\textbf{DNN inference on Microcontrollers.} 
STMicroelectronics has introduced X-CUBE-AI~\cite{xcubeai}, an expansion pack designed to streamline the deployment of high-level deep learning models, including 32-bit floating point and 8-bit quantized models, onto low-end STM32 microcontrollers.
TinyEngine~\cite{mcunet} which builds upon the CMSIS-NN~\cite{cmsis} and its software stack tailored for inference on ARM Cortex-M devices, integrates numerous optimization strategies.
These optimizations are aimed at enhancing inference speed and minimizing memory footprint, resulting in superior performance compared to aforementioned frameworks across several benchmarks.
Notably, the operations used within this framework are model-specific and thus the generated code is fully specialized to accommodate the models obtained through their NAS approach.
On the other hand, CMiX-NN~\cite{cmix}, a mixed low-precision inference library for low bit-width Quantized Networks~\cite{quant:tinyml}, tries to minimize memory requirements, by enabling aggressive and arbitrary quantization to effectively deploy CNNs on tiny MCUs.
Finally, MicroTVM~\cite{microtvm} is an open-source deep learning compiler stack (TVM) that provides a set of tools and libraries to optimize and deploy similarly DNNs across MCUs.

\textbf{Neural Network Model Optimization.}
An active research field explores ways to create efficient network models capable of running on small, resource-limited IoT devices.
Some approaches focus on approximating the model's architecture by prunning trainable parameters of the network~\cite{prun:survey22, benbaki2023fast,prun:tinyml} and in some cases they also totally remove less crucial channels from convolutional layers~\cite{chprune}, or replace the entire layers with smaller sub-layers~\cite{compress:tinyml}.
On the other hand, others employ NAS~\cite{nascnn,nas:survey} as a method to lower complexity and effectively design neural networks 
specifically for edge devices.

\orange{
Our work distinguishes from existing state-of-the-art works and can be classified alongside the frameworks listed in Table~\ref{tab:related}, since these frameworks share a common focus on optimizing the inference of trained DNNs on microcontrollers and do not target solely on the modification of the model's architecture or pre-training optimization/approximation approaches.
This Table provides a qualitative comparison of the related frameworks in the field of resource-constrained DNN inference, highlighting the key differences left unexplored in these works.
In brief, while X-CUBE-AI stands as a robust commercial tool, its orthogonality with other software techniques is limited due to its fixed quantization schemes and, thus, the improvements in latency are intricately linked to the optimizations inherent in the tool.
Moreover, TinyEngine presents models with various trade-offs between accuracy and latency. 
However, the absence of approximate optimizations and an efficient utilization of the targeted MCU prevent from finely tuned accuracy compromises that could lead to even more significant speedups.
Despite the distinctive features outlined in Table~\ref{tab:related}, in Section~\ref{sec:comp} we also evaluate our work against the listed frameworks and tools.
}

